A Scalable and Generalizable Pathloss Map Prediction

Large-scale channel prediction, i.e., estimation of the pathloss from geographical/morphological/building maps, is an essential component of wireless network planning. Ray tracing (RT)-based methods have been widely used for many years, but they require significant computational effort that may become prohibitive with the increased network densification and/or use of higher frequencies in B5G/6G systems. In this paper, we propose a data-driven, model-free pathloss map prediction (PMP) method, called PMNet. PMNet uses a supervised learning approach: it is trained on a limited amount of RT (or channel measurement) data and map data. Once trained, PMNet can predict pathloss over location with high accuracy (an RMSE level of $10^{-2}$) in a few milliseconds. We further extend PMNet by employing transfer learning (TL). TL allows PMNet to learn a new network scenario quickly (x5.6 faster training) and efficiently (using x4.5 less data) by transferring knowledge from a pre-trained model, while retaining accuracy. Our results demonstrate that PMNet is a scalable and generalizable ML-based PMP method, showing its potential to be used in several network optimization applications.

==> table/parameter_network_pmnet_parameter.tex <==
% \begin{tabular} {l l}
% \toprule[1.5pt]
% \textit{\textbf{Parameter}} & \textit{\textbf{}} \\
% \cmidrule(lr){1-2}
\begin{tabular}{c c}
\toprule[1.5pt]
\textit{Parameter} & \textit{Values}\\ 
\cmidrule(lr){1-2}
% \midrule[.7pt] 
Number of blocks            & $[3, 3, 27, 3]$          \\ 
Atrous rates                & $[6, 12, 18]$          \\ 
Multi-grids                 & $[1, 2, 4]$ or None          \\ 
Output stride               & $16$ or $8$   \\ 
\bottomrule[1.5pt]
\end{tabular}
